Content Delivery over Broadcast Erasure Channels with Distributed Random Cache

We study the content delivery problem between a transmitter and two receivers through erasure links, when each receiver has access to some random side-information about the files requested by the other user. The random side-information is cached at the receiver via the decentralized content placement. The distributed nature of receiving terminals may also make the erasure state of two links and indexes of the cached bits not perfectly known at the transmitter. We thus investigate the capacity gain due to various levels of availability of channel state and cache index information at the transmitter. More precisely, we cover a wide range of settings from global delayed channel state knowledge and a non-blind transmitter (i.e. one that knows the exact cache index information at each receiver) all the way to no channel state information and a blind transmitter (i.e. one that only statistically knows cache index information at the receivers). We derive new inner and outer bounds for the problem under various settings and provide the conditions under which the two match and the capacity region is characterized. Surprisingly, for some interesting cases the capacity regions are the same even with single-user channel state or single-user cache index information at the transmitter.

==> ConverseDD.tex <==
\appendices


\section{Converse Proof of $\mathcal{C}^\mathrm{non-blind}_\mathrm{DD}$ in Theorem~\ref{THM:Capacity_Out_BIC_Delayed}}
\label{Section:DDBounds}

%{\color{red} From the rejected paper, needs to include non-homogeneous by Alireza.}

The derivation of the outer-bounds on the individual rates is straightforward and thus omitted. In fact, it is well established that the capacity of a point-to-point erasure channel with erasure probability $\delta_i$ is $\lp 1 - \delta_i \rp$. In what follows, we derive
\begin{align}
\label{Eq:ConverseBound}
\beta_1^{\mathrm{delayed}} R_1 + R_{2} \leq \left( 1 - \delta_2 \right),
\end{align}
where as indicated in \eqref{Eq:Beta_Delayed}, we have
\begin{align}
\label{Eq:beta1recap}
\beta_1^{\mathrm{delayed}} = \epsilon_2 \frac{1-\delta_2}{1-\delta_1\delta_2}.
\end{align}
The derivation of the other bound would follow by simply changing user IDs $1 \leftrightarrow 2$.



Suppose rate-tupe $\lp R_1, R_2 \rp$ is achievable. We enhance receiver $\msf{Rx}_1$ by providing the entire $W_2$ to it, as opposed to $W_{2|1}$, and we note that this cannot reduce the rates. Then, we have
\begin{align}
n &\left( \beta_1^{\mathrm{delayed}} R_1 + R_2 \right) = \beta_1^{\mathrm{delayed}} H(W_1) + H(W_2) \nonumber \\
& \overset{(a)}= \beta_1^{\mathrm{delayed}} H(W_1|W_2, G^n) + H(W_2|W_{1|2},G^n) \nonumber \\
& \overset{(\mathrm{Fano})}\leq \beta_1^{\mathrm{delayed}} I(W_1;Y_1^n|W_2,G^n) + I(W_2;Y_2^n|W_{1|2},G^n) + n \upxi_n \nonumber \\
& = \beta_1^{\mathrm{delayed}} H(Y_1^n|W_2,G^n) - \beta_1^{\mathrm{delayed}} \underbrace{H(Y_1^n|W_1,W_2,G^n)}_{=~0} \nonumber \\
& \quad + H(Y_2^n|W_{1|2},G^n) - H(Y_2^n|W_{1|2},W_2,G^n) + n \upxi_n \nonumber \\
& \overset{(b)}\leq H(Y_2^n|W_{1|2},G^n) + 2n \upxi_n \nonumber \\
& \overset{(c)}\leq n \left( 1 - \delta_2 \right) + 2\upxi_n,
\end{align}
where $\upxi_n \rightarrow 0$ as $n \rightarrow \infty$; $(a)$ follows from the independence of the messages and captures the enhancement of receiver $\msf{Rx}_1$; $(b)$ follows from Lemma~\ref{Lemma:Leakage_BIC} below; and $(c)$ holds since
\begin{align}
H(Y_2^n|W_{1|2},G^n) \leq H(Y_2^n|G^n) \leq \sum_{t=1}^{n}{ H(Y_2[t]|G^n)} = \sum_{t=1}^{n}{(1-\delta_2)H(X[t]|G^n)} \leq n(1-\delta_2).
\end{align}
Dividing both sides by $n$ and let $n \rightarrow \infty$, we get \eqref{Eq:ConverseBound}.

\begin{lemma}
\label{Lemma:Leakage_BIC}
For the two-user erasure broadcast channel with channel feedback and side information at the receivers as described in Section~\ref{Section:Problem_BIC}, and $\beta_1^{\mathrm{delayed}}$ given in (\ref{Eq:beta1recap}), we have
\begin{align}
\beta_1^{\mathrm{delayed}} H\left( Y_1^n | W_2, G^n \right) - H(Y_2^n|W_{1|2},W_2,G^n) \leq n \upxi_,
%H\left( Y_2^n | W_{1|2}, W_2, G^n \right) + n \upxi_n \geq \frac{1}{\beta} H\left( Y_1^n | W_2, G^n \right),
\end{align}
where $\upxi_n \rightarrow 0$ as $n \rightarrow \infty$.
\end{lemma}

%%%%ALIREZA%%%%

\begin{proof}
For time instant $t$ where $1 \leq t \leq n$, we have
\begin{align}
& H\left( Y_2[t] | Y_2^{t-1}, W_{1|2}, W_2, G^t \right) \\
& \quad = \lp 1 - \delta_2 \rp H\left( X[t] | Y_2^{t-1}, W_{1|2}, W_2, G_{2}[t] = 1,  G^{t-1} \right) \nonumber \\
& \quad \overset{(a)}= \lp 1 - \delta_2 \rp H\left( X[t] | Y_2^{t-1}, W_{1|2}, W_2, G^t \right) \nonumber \\
& \quad \overset{(b)}\geq \lp 1 - \delta_2 \rp H\left( X[t] | Y_1^{t-1},Y_2^{t-1}, W_{1|2}, W_2, G^t \right) \nonumber \\
& \quad = \frac{1 - \delta_2}{1 - \delta_1\delta_2} H\left( Y_1[t], Y_2[t] | Y_1^{t-1},Y_2^{t-1}, W_{1|2}, W_2, G^t \right), \end{align}
where $(a)$ holds since $X[t]$ is independent of the channel realization at time instant $t$; $(b)$ follows from the fact that conditioning reduces entropy. Next, since the transmit signal at time instant $t$ is independent of future channel realizations, we get
\begin{align}
\label{Eq:withSideInfo}
& H\left( Y_2^n | W_{1|2}, W_2, G^n \right)  \\
& \geq \frac{1 - \delta_2}{1 - \delta_1\delta_2} H\left( Y_1^n, Y_2^n | W_{1|2}, W_2, G^n \right) \geq \frac{1 - \delta_2}{1 - \delta_1\delta_2} H\left( Y_1^n | W_{1|2}, W_2, G^n \right). \nonumber
\end{align}
We note that
\begin{align}
H\left( Y_1^n | W_1, W_2, G^n \right) = 0,
\end{align}
and
\begin{align}
H\left( W_1 | Y_1^n, W_2, G^n \right) \leq n \upxi_n,
\end{align}
combining these with \eqref{Eq:MessageSplitting}, we get
\begin{align}
\label{Eq:RemovingSideInfo}
H\left( Y_1^n | W_{1|2}, W_2, G^n \right)  \geq \epsilon_2 H\left( Y_1^n | W_2, G^n \right) - n \upxi_n.
\end{align}
Finally, from \eqref{Eq:withSideInfo} and \eqref{Eq:RemovingSideInfo}, we obtain
\begin{align}
H\left( Y_2^n | W_{1|2}, W_2, G^n \right) + n \upxi_n \geq \beta_1^{\mathrm{delayed}} H\left( Y_1^n | W_2, G^n \right).
\end{align}
This completes the proof of Lemma~\ref{Lemma:Leakage_BIC}, and thus, the optimality proof.
\end{proof}
